Habitat-Web: Learning Embodied Object-Search Strategies from Human Demonstrations at Scale

We present a large-scale study of imitating human demonstrations on tasks that require a virtual robot to search for objects in new environments -- (1) ObjectGoal Navigation (e.g. 'find & go to a chair') and (2) Pick&Place (e.g. 'find mug, pick mug, find counter, place mug on counter'). First, we develop a virtual teleoperation data-collection infrastructure -- connecting Habitat simulator running in a web browser to Amazon Mechanical Turk, allowing remote users to teleoperate virtual robots, safely and at scale. We collect 80k demonstrations for ObjectNav and 12k demonstrations for Pick&Place, which is an order of magnitude larger than existing human demonstration datasets in simulation or on real robots. Second, we attempt to answer the question -- how does large-scale imitation learning (IL) (which hasn't been hitherto possible) compare to reinforcement learning (RL) (which is the status quo)? On ObjectNav, we find that IL (with no bells or whistles) using 70k human demonstrations outperforms RL using 240k agent-gathered trajectories. The IL-trained agent demonstrates efficient object-search behavior -- it peeks into rooms, checks corners for small objects, turns in place to get a panoramic view -- none of these are exhibited as prominently by the RL agent, and to induce these behaviors via RL would require tedious reward engineering. Finally, accuracy vs. training data size plots show promising scaling behavior, suggesting that simply collecting more demonstrations is likely to advance the state of art further. On Pick&Place, the comparison is starker -- IL agents achieve ${\sim}$18% success on episodes with new object-receptacle locations when trained with 9.5k human demonstrations, while RL agents fail to get beyond 0%. Overall, our work provides compelling evidence for investing in large-scale imitation learning. Project page: https://ram81.github.io/projects/habitat-web.

==> RebuttalTemplate.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \usepackage[rebuttal]{cvpr}
% \input{imports}


% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}

% % some bib space saving hacks
% \usepackage{biblatex}
% \addbibresource{strings.bib}
% \addbibresource{main.bib}
% \renewcommand*{\bibfont}{\footnotesize}


% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% % \usepackage[pagebackref,breaklinks,colorlinks,bookmarks=false]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% % If you wish to avoid re-using figure, table, and equation numbers from
% % the main paper, please uncomment the following and change the numbers
% % appropriately.
% %\setcounter{figure}{2}
% %\setcounter{table}{1}
% %\setcounter{equation}{2}

% % If you wish to avoid re-using reference numbers from the main paper,
% % please uncomment the following and change the counter for `enumiv' to
% % the number of references you have in the main paper (here, 6).
% %\let\oldthebibliography=\thebibliography
% %\let\oldendthebibliography=\endthebibliography
% %\renewenvironment{thebibliography}[1]{%
% %     \oldthebibliography{#1}%
% %     \setcounter{enumiv}{6}%
% %}{\oldendthebibliography}


% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\cvprPaperID{4844} % *** Enter the CVPR Paper ID here
% \def\confName{CVPR}
% \def\confYear{2022}

% \begin{document}

% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{Learning Embodied Object-Search Strategies from 50k Human Demonstrations}

% \maketitle

% \input{sections/rebuttal/rebuttal_content}


% %%%%%%%%% REFERENCES
% \begingroup
% % \bibliographystyle{ieeetr}
% % \biboptions{sort&compress}
% % \bibliography{strings,main}
% \setlength\bibitemsep{0pt}
% \printbibliography[heading=none]
% \endgroup

% \end{document}


==> sections/main/baselines.tex <==
\section{Baselines}

% that takes an embedding of visual inputs (RGB and depth), instruction and action $(a_{t-1})$ executed at time step t-1, then predicts an action $a$.

% \ad{Two results we plan to demonstrate here are 1) compounding errors
% especially with a small set of demonstrations, and 2) a plot of behavior cloning
% performance~\vs dataset size, going from ${\sim}3k$ to ${\sim}15k$ demonstrations,
% where we expect compounding error issues to reduce with more data.}

% \ad{There is also a possibility that behavior cloning will work surprisingly well
% as we scale up data, in which case we might make that the primary focus of the
% paper instead of reward modeling.}

% % % % % % % % % % % % % % % OLD APPROACH WHEN THE FOCUS WAS REWARD MODELING.

% \subsection{RL with manually-specified rewards}
% \label{sec:rl_true}

% \begin{compactitem}
% \item The agent receives an exploration reward $r_{explore}$, a grab success
% reward $r_{grab}$ to encourage
% successfully picking up the object, a distance reward $r_{distance}$, a
% task success reward $r_{success}$.
% % \item To solve the pick and place task, we encourage the agent by giving a grab reward on first grab success for every episode.
% \item The exploration reward is based on visitation count as described in \cite{ye_iccv21}
% and incentivizes initial search behavior for the target object in the
% `pick and place` task.
% \item The distance reward is a function of the change in geodesic distance and
% has two phases -- 1) distance between the agent and the target object ($g[1]$)
% until the target object is picked up, and 2)  distance between the agent and the
% receptacle ($g[2]$) after the agent has picked up the target object.
% \end{compactitem}

% \begin{equation*}
% r_{total} = r_{explore} + r_{grab} + r_{distance} + r_{success}
% \end{equation*}

% \begin{equation*}
% r_{success} = 3.5 \quad \text{on success}
% \end{equation*}

% \begin{equation*}
% r_{grab} = 2.5 \quad \text{first grab success}
% \end{equation*}

% \begin{equation*}
% r_{distance} =
% \begin{cases}
%     \text{GeoDist}(s_{t}, g[1]) - \text{GeoDist}(s_{t+1}, g[1])& \text{if object not gripped},   \\

%     \text{GeoDist}(s_{t}, g[2]) - \text{GeoDist}(s_{t+1}, g[2])& \text{otherwise},   \\
% \end{cases}
% \end{equation*}

% \begin{equation*}
% r_{explore} =
% \begin{cases}
%     0.25 \times \frac{d^t}{v}& \text{if object not seen},   \\
%     0& \text{otherwise},   \\
% \end{cases}
% \end{equation*}

% % We also experiment with an
% % As searching for object is a sub task to complete and the describe visitation
% % based exploration was found helpful for ObjectNav task. In these experiments agent
% % gets an exploration reward $r_{explore}$ until the object is seen for the first
% % time in an episode. We can write the reward as

% % \begin{equation*}
% % r_{total} = r_{success} + r_{grab} + r_{distance} + r_{explore}
% % \end{equation*}


==> sections/rebuttal/rebuttal_content.tex <==
\noindent We thank reviewers for their feedback!
We are happy that they found the problem we study and our data collection infrastructure important (R1,2),
our dataset of human demonstrations orders of magnitude larger than prior datasets (R2,3),
the quantitative and qualitative analyses to be high quality (R1) and experiments extensive (R3).
We address specific comments below and will incorporate all feedback.

% the dataset is "pretty large in terms of human demonstrations" (R2,3) and is "compelling for future research" (R2), that our infrastructure is "important to collect human demonstrations" (R1,2). One primary concern was regarding the novelty and main findings being not that surprising or new.

\xhdr{\Rone{} Status of data collection.}
At the time of submission, we had collected a dataset of $40k$ \objnav demonstrations.
Since then, we have collected an additional $33k$, amounting to $73k$ for \objnav, and $85k$ total demonstrations (including \pickplace).
We are on track towards a dataset of $100k$ demonstrations. At $40k$
our dataset was already the largest by an order of magnitude; the expansion to $100k$ is simply 
to find a saturation point on performance. 

\begin{table}[h]
    \centering
    \resizebox{0.975\columnwidth}{!}{
        \begin{tabular}{@{}llrr@{}}
            \toprule
            & Team / Method & Success $(\mathbf{\uparrow})$ & SPL $(\mathbf{\uparrow})$ \\
            \midrule
            \rownumber & DD-PPO baseline~\cite{wijmans_iclr20} & $6.2\%$ & $2.1\%$ \\
            \rownumber & Red Rabbit (6-Act Base)~\cite{ye_iccv21} & $24.5\%$ & $6.4\%$ \\
            \rownumber & Red Rabbit (6-Act Tether)~\cite{ye_iccv21} & $21.1\%$ & $8.1\%$ \\
            \midrule
            \rownumber & IL w/ $40k$ Human Demos (in paper) & $24.4\%$ & $8.2\%$ \\
            \rownumber & IL w/ $45k$ Human Demos & $\mathbf{25.4}\%$ & $\mathbf{8.4}\%$ \\
            \bottomrule
            \end{tabular}
    }
    \vspace{5pt}
    \caption{ObjectNav results on Habitat \textsc{test-std}.}
    \label{tab:objnav_test}
    \vspace{-5pt}
\end{table}

\xhdr{\Rone{} (Updated) IL vs RL comparison.}
%gets lower success than RL on \objnav, even though RL doesn't require human annotations.}
% 
We trained an IL agent on $45k$ \objnav demonstrations,
achieving $25.4\%$ success and $8.4\%$ SPL,
an improvement of $0.9\%$ success over
% over IL on $40k$ episodes as reported in the paper.
% This outperforms
RL (Red Rabbit~\cite{ye_iccv21}). %See Tab.~\ref{tab:objnav_test}.
% We expect to have the full dataset of $100k$ demonstrations for \objnav in place by the final version.
% While we agree that IL on $40k$ demos is $0.1\%$ worse on success (and $1.8\%$ better on SPL!) than
% RL (Red Rabbit),
We expect the performance of IL to only increase as we train on the fully collected 
dataset. 
We also reiterate that \cite{ye_iccv21} is a highly engineered approach with
auxiliary loss functions and carefully-tuned rewards
% requiring substantial researcher hours (instead of data annotation hours)
compared to our IL setup without such bells and whistles.
% that the current baseline trained on $40k$ human demonstrations shows comparable results ($0.1\%$ worse Success and $1.8\%$ better SPL on \textsc{test-std} split) with RL counterpart (Red Rabbit). But we would like to point out that the Red Rabbit baseline includes a set of auxiliary tasks in addition to engineered exploration reward to achieve better performance on \objnav whereas our pipeline is much simpler (without bells and whistles) and it still shows comparable performance to SOTA. For \pickplace our simple IL baseline outperforms a RL baseline with engineered dense rewards by a large margin. Additionally, we demonstrate that it is worth investigating simpler pipelines for complex embodied tasks. \ram{I focused more on simplicity of our approach in this version. If we get SOTA before deadline I will update this section}.

% SOTA response
%Our approach trained on $50k$ demos achieves $X\%$ success and $Y\%$ SPL, outperforming prior RL-trained counterparts- $X\%$ better on success and $Y\%$ better on SPL %than RL (Red Rabbit). We would like to remind that Red Rabbit~\cite{ye_iccv21} is a highly engineered approach with auxiliary loss functions and carefully-tuned % exploration rewards compared to our IL architecture without such bells and whistles.
% compared to our IL architecture without such bells and whistles.
% \ram{Change response if we get SOTA before rebuttal deadline}.

\xhdr{\Rone{} Main findings not that surprising.}
We agree that our experiments help validate the common knowledge that IL is 
more sample-efficient than RL seen in other domains.
%At a high-level, we generally agree. 
But (a) this seems clearer in hindsight than when we started (hindsight bias), 
(b) in semantic navigation, the focus of the community has been on 
reinforcement learning and our work shows precisely how much data is necessary for IL to 
outperform RL (45k), which we could not have predicted. 
%We agree in hindsight, but to our knowledge, these results have not been demonstrated in goal-directed
%embodied navigation before.
%Finally, \cite{weihs_arxiv21, alfred} have previously investigated IL using heuristic experts, not with human demonstrations.
 
%And as noted in your review, these experiments help validate the common knowledge that IL is more sample-efficient than RL seen in other domains.
%
% that the main findings seem intuitive and obvious.
%
% We believe there is value in investigating how to learn object-search strategies from human demonstrations as it is difficult to engineer rewards for such strategies. The analysis in section 7 of our main paper shows that it is possible to learn these strategies with a simple pipeline. Additionally, the comparison of IL on shortest paths (row 3) ~\vs IL on human demonstrations (row 5) in Table. 1 of our supplementary material shows that training IL agents on human demonstrations is easier compared to experts with access to privileged information because of lower imitation gap.

% Visual Room rearrangement - \cite{weihs_arxiv21} ALFRED - \cite{alfred}

\xhdr{\Rone{} Include sensor ablations in main.}
Thanks! Will do.
% We will update the final version of the paper to include sensor ablations in main text.

\xhdr{\Rone{} Why not pre-train with IL and finetune with RL?}
Thanks for the suggestion! That is indeed the next step in this line of research that we
are looking to pursue.

\xhdr{\Rtwo{} No novelty in imitation learning experiments.}
Yes, this is by design. 
As a reminder, our primary goal is to quantify the value of human demonstrations
for training navigation agents.
%
Thus, as described in L188-192, we intentionally used off-the-shelf imitation learning with an agent architecture without
any bells or whistles to isolate the effect of the data. 
Such a simple IL agent (trained on $45k$ demos) outperforms the SOTA 
RL agent, %($0.3\%$ better on SPL and $0.9\%$ better on success on \objnav \textsc{test-std}, 
Table~\ref{tab:objnav_test}.
%
As observed by R1, \emph{The models introduced are relatively simple and thus we can equate most
of the performance to IL on the collected trajectories.}
%While these experiments might seem intuitive in hindsight, 
Most importantly, our experiments validate our Habitat-WebGL data
collection infrastructure and the associated dataset of human demonstrations
(1-2 orders of magnitude larger than prior works, L144-150).
%
We intend to publicly release both to fuel future research.

%\xhdr{\Rtwo{} Duplicate sentences in abstract and introduction.}
%Thanks, we will update these.

% \begin{compactenum}[\hspace{2pt}-]

% \item \textbf{Habitat-WebGL Infrastructure}. We build a reliable pipeline to collect human demonstrations at scale which can generalize to any task being studied in Habitat \cite{savva_iccv19} unlike other efforts \cite{embodiedqa,hahn_arxiv20} that built one-off data collection infrastructures.

% \item \textbf{Largest dataset of human demonstrations for embodied tasks}. We collect a dataset of total $Xk$ human demonstrations which is an order magnitude larger than existing human demonstrations in simulation and 2 orders magnitude larger than datasets on real robots. Our dataset illustrates rich diverse object-search strategies to solve the tasks. This dataset enables future research to learn human-like object-search stratgies using IRL and IL methods.

% \item \textbf{Comparison of large-scale IL with large-scale RL}. Using our large-scale dataset we find that IL (with no bells or whistles) is comparable to RL on \objnav and outperforms RL on \pickplace by a large margin. We establish that IL-trained agents learn efficient object-search strategies from humans demonstrations with a simple pipeline which is hard to induce in RL agents through dense reward engineering.

% \end{compactenum}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/dataset_stats/objectnav_action_histogram.png}
    \vspace{5pt}
    \caption{ Action histograms for \objnav human demonstrations~\vs shortest paths.}
    \label{fig:objectnav_stats}
    \vspace{-10pt}
\end{figure}

\xhdr{\Rthree{} Human demonstrations dataset is biased. Fig. 3c shows most goals can be achieved with move forward.}

No. The reviewer is drawing a mistaken inference. 
Fig. 3c in paper (reproduced in \figref{fig:objectnav_stats})
shows action histograms for human demonstrations~\vs shortest paths. 
\moveforward is the most popular action but this \emph{does not mean that a forward-only 
agent would succeed at the task}. 
Specifically, we evaluated two forward-only agents:
\begin{compactenum}[\hspace{2pt}-]
    \item \textbf{\moveforward agent with oracle \stopac}. This agent executes only \moveforward actions until it reaches within success distance (\ie $1.0$m) of the goal and then executes a \stopac action using an oracle \stopac sensor. This achieves $1.0\%$ success, $0.7\%$ SPL on \objnav-\textsc{VAL}.
    \item \textbf{\moveforward agent with oracle \turnac and \stopac}. The agent first orients itself at
    its starting position towards the direction of the closest goal object using an oracle \turnac sensor and executes only \moveforward actions until it reaches within success distance (\ie $1.0$m) of the goal.
    It then executes a \stopac action using an oracle \stopac sensor. This achieves $1.6\%$ Success and $1.2\%$ SPL.
\end{compactenum}

As we can see, both agents (even with oracular components) utterly fail. Thus most goals are \emph{not} achievable using \moveforward actions. And data pruning is not needed. 


%Fig. 3c in the paper (reproduced in \figref{fig:objectnav_stats})
%shows action histograms for human demonstrations~\vs shortest paths.
A bias towards \moveforward is expected in these navigation trajectories:
% 
1) \moveforward is the only action that causes agent displacement.
The other actions -- \turnleft, \turnright, \lookup, \lookdown~-- only
affect agent orientation.
% 
2) These house layouts
often have long corridors and large rooms to navigate through.


% \ram{Should we start by saying "We disagree with this..."?}Please note that Fig. 3(c) in the main paper shows comparison of action histograms for human demonstrations~\vs shortest paths. We agree that the dataset has a bias for \moveforward action but the \objnav task is not solvable by just learning to \moveforward. To demonstrate this, we compare the performance for two oracle forward-only agents on \objnav \textsc{VAL} split.

% Additionally, we would also like to point out Fig. 4 from our supplementary material. The figure visualizes multiple human demonstrations for \objnav from same start position and searching for same goal. This figure shows the inter-human variance in the trajectories and demonstrates that there is quite a bit of diversity in navigation trajectories across humans.


\xhdr{\Rthree{} Dataset postprocessing not mentioned.}
% Thanks for the suggestion!
% We will include dataset postprocessing details in the main paper.
The only postprocessing we did was to filter out demonstrations that take more than $500$ steps
to succeed on \objnav (L367, ${\sim}12\%$ episodes) and more than $1500$ steps on \pickplace (L466, ${\sim}15\%$ episodes).
We will make this clearer. Thanks!
% When using the the full dataset of human demonstrations we see $X\%$ drop in success rate on \objnav and $Y\%$ drop in success rate on \pickplace. \ram{Update numbers}. We chose the threshold for filtering out demonstrations based on the maximum number steps allowed for each task.

% \xhdr{\Rone{}\Rtwo{} Dataset contribution not indicated.} We have indicated dataset as one of the contribution of the paper in the submission form and we will be releasing the full dataset with final paper.


==> space_saver.tex <==
% A collection of dubious space saving macros
%\setlength{\parindent}{0cm}
%\parskip=2pt
\abovedisplayskip 3.0pt plus2pt minus2pt%
\belowdisplayskip \abovedisplayskip
\renewcommand{\baselinestretch}{1} % only use this one in emergencies

%Section spacing
\newcommand{\csection}[1]{
    \vspace{-0.08in}
    \section{#1}
    \vspace{-0.08in}
}

\newcommand{\csubsection}[1]{
    \vspace{-0.08in}
    \subsection{#1}
    \vspace{-0.08in}
}

\newcommand{\csubsubsection}[1]{
    \vspace{-0.06in}
    \subsubsection{#1}
    \vspace{-0.05in}
}


%caption/figure spacing
\setlength{\floatsep}{1ex plus 0ex minus 0.5ex}
%\setlength{\textfloatsep}{0ex plus 0ex minus 0ex}
%\setlength{\abovecaptionskip}{0ex plus 0ex minus 0ex}
\setlength{\belowcaptionskip}{0ex plus 0ex minus 0.5ex}
